Test-Time Adaptation with SaLIP: A Cascade of SAM and CLIP for Zero shot Medical Image Segmentation

The Segment Anything Model (SAM) and CLIP are remarkable vision foundation models (VFMs). SAM, a prompt driven segmentation model, excels in segmentation tasks across diverse domains, while CLIP is renowned for its zero shot recognition capabilities. However, their unified potential has not yet been explored in medical image segmentation. To adapt SAM to medical imaging, existing methods primarily rely on tuning strategies that require extensive data or prior prompts tailored to the specific task, making it particularly challenging when only a limited number of data samples are available. This work presents an in depth exploration of integrating SAM and CLIP into a unified framework for medical image segmentation. Specifically, we propose a simple unified framework, SaLIP, for organ segmentation. Initially, SAM is used for part based segmentation within the image, followed by CLIP to retrieve the mask corresponding to the region of interest (ROI) from the pool of SAM generated masks. Finally, SAM is prompted by the retrieved ROI to segment a specific organ. Thus, SaLIP is training and fine tuning free and does not rely on domain expertise or labeled data for prompt engineering. Our method shows substantial enhancements in zero shot segmentation, showcasing notable improvements in DICE scores across diverse segmentation tasks like brain (63.46%), lung (50.11%), and fetal head (30.82%), when compared to un prompted SAM. Code and text prompts are available at: https://github.com/aleemsidra/SaLIP.

==> sec/2_formatting.tex <==
% % \section{Experiments}
% % \label{sec:formatting}
% % To evaluate the performance of SAM-CLIP-SAM we performed
% % both qualitative and quantitative experiments on four benchmark
% % colonoscopy datasets:
% % \subsubsection{Implementaion Detail}

% % \subsubsection{Ablation on prompt method}
% % \begin{itemize}
% %     \item \textbf{CC359} \ref{souza2018open}: 
% % \end{itemize}

% % We evaluate our approach on Calgary-Campinas (CC359)
% % dataset [26], a multi-vendor (GE, Philips, Siemens), multifield strength (1.5, 3) magnetic resonance (MR) T1-weighted
% % volumetric brain imaging dataset. It has six different domains
% % and contains 359 3D brain MR image volumes, primarily focused on the task of skull stripping.
% % All text must be in a two-column format.
% % The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% % Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% % The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% % The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% % On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% % for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% % page.

% % %-------------------------------------------------------------------------
% % \subsection{Margins and page numbering}

% % All printed material, including text, illustrations, and charts, must be kept
% % within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% % high.
% % %
% % Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% % The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% % The \LaTeX\ template takes care of this when used properly.



% % %-------------------------------------------------------------------------
% % \subsection{Type style and fonts}

% % Wherever Times is specified, Times Roman may also be used.
% % If neither is available on your word processor, please use the font closest in
% % appearance to Times to which you have access.

% % MAIN TITLE.
% % Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% % The title should be in Times 14-point, boldface type.
% % Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% % do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% % Leave two blank lines after the title.

% % AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% % and printed in Times 12-point, non-boldface type.
% % This information is to be followed by two blank lines.

% % The ABSTRACT and MAIN TEXT are to be in a two-column format.

% % MAIN TEXT.
% % Type main text in 10-point Times, single-spaced.
% % Do NOT use double-spacing.
% % All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% % Make sure your text is fully justified---that is, flush left and flush right.
% % Please do not place any additional blank lines between paragraphs.

% % Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% % Short captions should be centred.

% % \noindent Callouts should be 9-point Helvetica, non-boldface type.
% % Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% % FIRST-ORDER HEADINGS.
% % (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% % SECOND-ORDER HEADINGS.
% % (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% % If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% % %-------------------------------------------------------------------------
% % \subsection{Footnotes}

% % Please use footnotes\footnote{This is what a footnote looks like.
% % It often distracts the reader from the main flow of the argument.} sparingly.
% % Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% % If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% % Use Times 8-point type, single-spaced.


% % %-------------------------------------------------------------------------
% % \subsection{Cross-references}

% % For the benefit of author(s) and readers, please use the
% % {\small\begin{verbatim}
% %   \cref{...}
% % \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% % This will automatically insert the appropriate label alongside the cross-reference as in this example:
% % \begin{quotation}
% %   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
% %   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
% %   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% % \end{quotation}
% % If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% % {\small\begin{verbatim}
% %   \Cref{...}
% % \end{verbatim}}
% % command. Here is an example:
% % \begin{quotation}
% %   \Cref{fig:onecol} is also quite important.
% % \end{quotation}

% % %-------------------------------------------------------------------------
% % \subsection{References}

% % List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% % When referenced in the text, enclose the citation number in square brackets, for
% % example~\cite{Authors14}.
% % Where appropriate, include page numbers and the name(s) of editors of referenced books.
% % When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% % If you use the template as advised, this will be taken care of automatically.

% % \begin{table}
% %   \centering
% %   \begin{tabular}{@{}lc@{}}
% %     \toprule
% %     Method & Frobnability \\
% %     \midrule
% %     Theirs & Frumpy \\
% %     Yours & Frobbly \\
% %     Ours & Makes one's heart Frob\\
% %     \bottomrule
% %   \end{tabular}
% %   \caption{Results.   Ours is better.}
% %   \label{tab:example}
% % \end{table}

% % %-------------------------------------------------------------------------
% % \subsection{Illustrations, graphs, and photographs}

% % All graphics should be centered.
% % In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% % Instead use
% % {\small\begin{verbatim}
% %   \centering
% % \end{verbatim}}
% % at the beginning of your figure.
% % Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% % Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% % Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% % You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% % When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% % {\small\begin{verbatim}
% %    \usepackage{graphicx} ...
% %    \includegraphics[width=0.8\linewidth]
% %                    {myfile.pdf}
% % \end{verbatim}
% % }


% % % %-------------------------------------------------------------------------
% % % \subsection{Color}

% % % Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% % % If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% % % Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.



% \section{Introduction}
% \label{sec:intro}
% The utilization of Vision-Foundation models (VFMs) has become increasingly prominent
% in various vision-related tasks, predominently due to their zero-shot transfer capabilities ot the various downstream tasks. The Segment Anything Model (SAM) ~\cite{kirillov2023segment} and CLIP ~\cite{radford2021learning} have showcased remarkable generalization capabilities in segmentation and recognition, respectively. SAM, in particular, has been trained with a massive dataset of mask labels, making it highly adaptable to a wide range of downstream tasks through interactive prompts. SAM can be utilized to either segment everything in an image or segment specific region based on the prompts given as shown in ~\cref{fig:sam_modes}. SAM has shown impressive results in a broad range of natural imaging, it has been proven to lack equal advantages when directly applied in medical domains ~\cite{mazurowski2023segment}, ~\cite{deng2023segment},~\cite{zhou2023can}, ~\cite{hu2023sam}.  On the other hand, CLIP’s training with billions of text-image pairs has given it an unprecedented ability in zero-shot visual recognition.
% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=1\linewidth]{images/sam modes.png}

%    \caption{SAM modes. (a) Input  (b) SAM everything mode (c-d) SAM promptable mode: bbox prompt, 1 point and 3 points (these prompts are generated from ground truth).}

%    \label{fig:sam_modes}
% \end{figure}
% Both SAM and CLIP have shown remarkable zero-shot transfer capabilities in various downstream tasks in the natural imaging. However, their unified  potential in the challenging medical imaging domain has not yet been explored. 

% % This works presents an in-depth exploration of integrating SAM and CLIP into a simple unified framework for organ segmentation. 

% % Several recent studies, including ~\cite{deng2023segment}, ~\cite{huang2024segment}, ~\cite{huang2024segment}, ~\cite{hu2023sam}, \cite{mattjie2023exploring}, \cite{mohapatra2023brain} have evaluated SAM’s capability on different medical image segmentation tasks in the context of zero-shot transfer. 
% While SAM  offers considerable advantages, it also has inherent limitations to their application in medical image segmentation. SAM, for instance relies on the prompts to segment specific regions. This prompt engineering requires domain expertise and manual intervention. However, in the medical imaging, its challenging due to scarcity and availability of high-quality labeled medical data. To address this, a few studies have integrated SAM with other foundation models such as GroundingDINO ~\cite{liu2023grounding} and  YOLOV8 ~\cite{Jocher_Ultralytics_YOLO_2023} to generate prompts ~\cite{pandey2023comprehensive}, ~\cite{biswas2023polyp} to get bounding box prompts for regions of interest (ROI).  However, these models rely on a combination of images and specific text prompts, thus prompt engineering issue still remains. 
%  % However, for effective ROI detection,  these models need images along-with relevant text prompts. They cannot be directly applied to medical images and require training and fine-tuning of prompts for ROI detection. Thus, despite their integration with SAM, the challenge of domain expertise for  prompt generation still persists with an added overhead of additional training.
 
% Furthermore, although SAM's capability of automatically segmenting everything in the image is appealing, however its application to medical imaging faces challenges. One of the main challenges lies in the inherent variability of segmentation tasks. For example, given a liver cancer CT image, the segmentation task can vary depending on the specific clinical scenario. 
% One clinician may be focused on segmenting the liver tumor, whereas another may require segmentation of the entire liver along with surrounding organs. Additionally,  clinicians are primarily interested to analyze specific anatomical organs such as the liver, kidneys, spleen, and lesions etc. It becomes challenging to discern and focus on regions of interest amidst the growing number of segmented areas. Thus, such challenges impedes the direct application of SAM to medical image segmentation. 
% % Medical image segmentation is integral component of numerous medical image analysis tasks and computer-aided diagnoses \cite{mazurowski2023segment}. The scarcity of labeled data in medical imaging poses challenges, hindering model generalization and performance. 
%  % Supervised medical image segmentation relies on labeled data to accurately identify structures within images. However, scarcity of labeled data in medical imaging poses challenges, hindering model generalization and performance. 
% % The Vision-Language Models (VLMs) have led to significant transformation within the domain of vision tasks ~\cite{li2021align}, ~\cite{radford2021learning}, ~\cite{alayrac2022flamingo}. VLMs are trained on the extensive amount of data, thereby eliminating the need for supervised training labels  and can be transferred to several downstream tasks. 
% % One prominent vision foundation model is Meta's Segment Anything Model (SAM). 
% % Recently, the Segment Anything Model (SAM), a vision foundation model trained on over 1 billion masks, has demonstrated impressive zero-shot segmentation capabilities across various vision tasks \cite{kirillov2023segment}. SAM is a universal promptable segmentation foundation model, trained predominantly on natural images \cite{kirillov2023segment}. It has two different modules: everything  and prompatable . The \textit{everything module} can provide an exceptionally thorough prediction of almost any object or part within images as shown in \cref{fig:sam_modes}(b). The \textit{promptable module} is designed to segment an object via prompts, which can be a single point, a set of points, a bounding box, or text \cref{fig:sam_modes}(c-e). 

% % SAM-based medical image segmentation research can be divided into two categories. The first line of research focuses typically involve fine-tuning either SAM's pre-trained image encoder or mask decoder \cite{ma2024segment}, ~\cite{zhang2023customized}, ~\cite{wu2023medical}. Despite the potential, it's essential to acknowledge that such methods need substantial volume of data for fine-tuning, which is not readily available in the medical field.
% % % Although these methods achieve satisfactory results for segmenting everything, 
% % The second line of research focuses to evaluate the performance of zero-shot segmentation by prompting SAM to get specific object segmentation.  Several recent studies, including ~\cite{deng2023segment}, ~\cite{huang2024segment}, ~\cite{huang2024segment}, ~\cite{hu2023sam}, \cite{mattjie2023exploring}, \cite{mohapatra2023brain} have evaluated SAM’s capability on different medical image segmentation tasks in the context of zero-shot transfer.  However, manually and accurately prompting SAM from scratch will be time-consuming and inefficient for medical professionals.
% % While both SAM's everything and promptable modules offer considerable advantages, they also have inherent limitations, particularly in the context of medical imaging. The former, for instance, is exceptionally good with part based segmentation but it lacks semantic knowledge about these regions ~\cite{yuan2024open}. Moreover, in certain cases, it may produce masks for irrelevant regions. Thus it has limited applicability in medical domain, where the clinicians are primarily interested to analyze specific anatomical regions such as the liver, kidneys, spleen, and lesions etc. It becomes challenging to discern and focus on regions of interest amidst the growing number of segmented areas. On the contrary, the latter, has wider applications in medical imaging due to its ability to segment specific regions. It's performance greatly depends on the type of prompt utilized. However, the domain expert annotations proves to be both costly and challenging to obtain within the medical domain, thereby impeding the scalability promoptable mode.
% % To address this, a few studies have integrated SAM with other foundation models such as GroundingDINO ~\cite{liu2023grounding} and  YOLOV8 ~\cite{Jocher_Ultralytics_YOLO_2023} to generate prompts ~\cite{pandey2023comprehensive}, ~\cite{biswas2023polyp}. The primary goal of GroundingDINO ~\cite{liu2023grounding} and YOLOV8 ~\cite{Jocher_Ultralytics_YOLO_2023} in this context is to detect approximate boundary boxes around the regions of interest (ROI) in medical images. However, for effective ROI detection, both of these models need images along-with relevant text prompts. They cannot be directly applied to medical images and require training and fine-tuning of prompts for ROI detection. Thus, despite their integration with SAM, the challenge of domain expertise for  prompt generation still persists with an added overhead of additional training.
% To address the aforementioned challenges,  we leverage the combined capabilities of SAM and CLIP,  and introduce a unified framework called SAM-CLIP-SAM, for zero-shot organ segmentation. Intially, our framework,  employs SAM to automatically segment every part within the image. SAM provides exhaustive segmentation, however the resulting masks lack semantic labels. To extract the relevant ROI mask from pool of generated masks, we first crop the original image according to these masks. This set of cropped regions is passed to CLIP. CLIP employing visually descriptive (VDT) sentences related to the target organ, retrieves the corresponding crop in a zero-shot manner ~\cite{maniparambil2023enhancing}. The VDT prompts for CLIP are generated via GPT-3.5. Finally, retrieved ROI mask is used for bounding box prompt generation, which is eventually use to prompt SAM to guide the specific organ segmentation. Hence, our framework is  completely independent of domain expertise or labeled data for prompt engineering. By combining the strengths of SAM and CLIP, our method is effectively performs zero medical organ segmentation. We conduct experiments across three diverse medical imaging datasets encompassing MRI scans, ultrasound and X-ray images. 
% Our contributions can be summarized as follows:
% \begin{itemize}
%     \item We propose a simple and straight-forward unified framework that leverages the strength of both SAM's everything and promptable modules for zero-shot medical image segmentation
%     \item We propose to employ SAM's everything module to aid the prompt generation in a zero shot-manner for medical image segmentation for SAM promptable module. To best of our knowledge we are first to explore the use of everything module to aid the prompt generation for SAM. 

%     \item Our proposed method adapts SAM fully at test time for medical imagining segmentation, thereby alleviating the need of if training, fine-tuning strategies and domain expertise for prompt engineering.
% \end{itemize}
% % In this work, we address these challenges with a unified framework, leveraging  strengths of both modules within SAM. Firstly, we employ SAM's everything mode in a zero-shot fashion to obtain all the region proposals within the image, eliminating the need for extra models/additional training for this task. Next, to obtain ROIs, we crop the original image based on SAM's generated proposals. This pool of cropped regions is then fed to CLIP ~\cite{radford2021learning} to retrieve the crop corresponding to ROI in a zero-shot domain transfer. To alleviate domain expertise for prompt engineering for CLIP, we adopted the method proposed in ~\cite{maniparambil2023enhancing}, which uses GPT-4 to generate visually descriptive textual prompts for CLIP. Finally, we use the retrieved ROI, to create bounding box for this and use it to prompt SAM.  
% % We conduct experiments across three diverse medical imaging datasets encompassing MRI scans, ultrasound and X-ray images.
% % to aid the prompt generation for SAM promptable mode. Now the question is How can we adeptly identify Regions of Interest (ROI) from the array of proposals and leverage them to initiate SAM effectively? To bridge up this gap, 
% % How can we efficiently identify important areas from suggested options and use them to trigger SAM
% % Though t
% % However, a pertinent question remains: how do we effectively extract Regions of Interest (ROI) from the pool of proposals and utilize them to prompt SAM?
% % Our primary objective is to first harness SAM's everything mode to generate region proposals, then extract regions of Interest (ROI) from the pool of proposals, prompting it, and subsequently passe it through SAM's prompt encoder. SAM does not have semantic knowldge about region propsal, so to bridge up the up gap between SAM's distinct modules we propose to use CLIP. 
% % To bridge the gap between% Our primary goal is to leverage SAM to get the region proposals and then get ROI from set of SAM's generated region proposal, get the prompt for it and pass it to SAM's prompt encoder. 
% % Since SAM's everything module can propose an extremely exhaustive prediction of almost any part in the images. This eliminates the need of additional models for region detection. Rather, we aim to use these region propsals to get the relevant region. 
% % Secondly, SAM's promptable module  is effective in ROI segmentation based on the prompts given. .
% % Thus our objective is to harness the strength of SAM' everything mode to aid the prompt generation for SAM' promatalde mode. To bridge the gap between the two modules, we use CLIP. 
% % Our objective is to get ROI from these region proposals. a
% % Secondly, SAM's promptable module  is effective in ROI segmentation based on the prompts given. Our framework, harness the capability of SAM' everything module for regions prosoal to aid the prompt geenration for SAM's promatable mode. 
% % To bridge up the gap between the two distinct mode, we use CLIP. Intialy ,everything module generates region propsals for all the parts in the image. The image is cropped according to the region propsals and all these crops are passed to CLIP. 
% % all these regions are then forwarded to CLIP to retrive the ROI from the set of generated region propsals. The retrived crop 
% % eliminating the need for additional models to detect Regions of Interest (ROI) for prompt engineering. Secondly, SAM's promptable mode is effective in ROI segmentation based on the prompts given. % which uses both modules of SAM. Since, SAM's everything module can exhaustively segment every region. So, we do not need any additional models to detect ROI for prompt engineering . 
% % We propose to use SAM's everything module to aid the prompt generation for SAM' promptable mode. To bridge the two distinct components of SAM effectively, we use CLIP. 
% % Rather, we harness the SAM's region generation capability to aid prompt engineering. TO bridge the SAM's both module 
% % To bridge these two distinct modes of SAM, we use CLIP . First we geenrate region propsals for all the 
% % harnessing the capabilities of SAM's everything mode capability to exhaustively segment every region in the image to aid the process of genera
% % a) since SAM can exhasutively genrate region proposals with zero-shot manner, this elim
% % However, for ROI detection, both these models  alongwith the images require the relevant text prompts. They cannot be applied directly on the medical images and need both training and prompt tuning to generate pormpts for ROI. Thus, with the integration of these models with SAM, the issue of domain expertise for prompt issue still persists. Additionally, it adds extra overhead since these models cannot be directly applied to medical imaging and needs additional trainig to detect ROI. 
% % both with the inerboth these models, the issue of domain expertise for giving text prompts for these models persists. It adds an extra level of complexity since these models cannot be directly used for medical imaging and require few-shot training to detect relvanot roi. 
% % Our objective is  to ahrness am , training free
% % have leveraged alternative foundation models such as GroundingDINO ~\cite{liu2023grounding} and YOLOV8 ~\cite{Jocher_Ultralytics_YOLO_2023} to detect the objects within images and then use the detected bounidng . However, 
% % Zero-shot text-to-bbox approach for object detection.
% % To address these, several studies have used other foundation models like GroundingDINO and YOLOV8, for prompt engineering for SAM . 
% % However, both these models require textual prompts which have been manayly crafted.  
% % we aim to create a bridge between the individual capabilities of SAM. 
% % Generally,  ground truth  or domain expertise are used for prompt engineering. Thus, in medical imaging where the ground truth are
% % While these methods can effectively segment various elements in medical images, their practical application in medical imaging is limited due to the absence of specific semantic labels, as depicted in \cref{fig:sam_modes}(b). Clinicians need to focus on specific areas such as the liver, kidneys, spleen, and lesions and it becomes difficult to analyze specific regions among the growing number of segmented areas. Moreover, these methods still require substantial amount data for fine-tuning, which is not readily available in the medical field.
% % Such methods has wider application in medical field, where the objective is to analyze specific organ/disease. However, these methods rely on either ground truth data or domain expertise for prompt engineering.
% % To address the above stated issues related to SAM, we aim to use SAM everything mode to aid prompt engineering for SAM's promptable mode. B
% % The results show that SAM can generate satisfactory masks with sufficient high-quality prompts for certain datasets. However, still with this mode, the 
% % In this paper, we aim to utilize the region proposals from SAM to aid the process of prompt generation for SAM. 
% % These works suggesr that the  perfomance of SAM is highlight depedant on the prompts. 
% % our objective is how to get relevant mask from region prospals, and how to give prompts without manual inetrventuon.
% % since sam doesnot recognize, so to create a bridge between sam propssl and getting the relevant prompt, we propose to use CLIP for the relevant mask retirval and use it to prompt SAM.
% % The clinicians mainly  focus on specific meaningful region , e.g., the liver, kidneys, spleen, and lesions and the increasing number of segmented regions can significantly complicate the analysis of specific areas. Furthermore, although these methods yield satisfactory results for segmenting everything, they still need substantial data for fine-tuning, which is not readily available in the medical domain. 
% % they still require a significant amount of data for fine-tuning, which is often lacking in the medical field. Moreover, despite the potential of such methods,
% % While these methods yield satisfactory results for segmenting everything, they still need substantial data for fine-tuning, which is not readily available in the medical domain. Moreover, these approaches do not focus on a specific region of interest (ROI) segmentation. Rather, they highlight the potential of SAM for segmenting all the regions in the medical imaging.

% % how to better adapt SAM to segment everything in medical images. These methods fine-tune either the SAM's pre-trained image encoder or mask decoder while utilizing the default SAM's prompt encoder or keeping it frozen \cite{ma2024segment}, ~\cite{zhang2023customized}, ~\cite{wu2023medical}. Despite it potential, its usefulness is in medical imaging is limited ~\cite{ma2024segment} as the identified regions lack semantic labels as shown in \cref{fig:sam_modes} and and clinicians mainly focus on specific region , e.g., the liver, kidneys, spleen, and lesions. While these methods yield satisfactory results for sgementing everything, they still need substantial data for fine-tuning, which is not readily available in the medical domain. Moreover, these approaches do not focus on a specific region of interest (ROI) segmentation. Rather, they highlight the potential of SAM for segmenting all the regions in the medical imaging.
% % (b). Moreover, the  clinicians primarily need to focus on specific region in the images such as the liver, kidneys, spleen, lesions, etc. 
% % Thus to get the region of interstet prompts are require.
% % It has limited applications in in medical domain as these propsals have no semantic labels and clinicians mainly focus on meaningful ROIs in clinical scenarios, e.g., the liver, kidneys, spleen, and lesions 
% % .  everything mode for medical image segmentation and use the defaul prompts of SAM. The methods works have fine tune SAM on medical image segmentation using traditional, LoRA based parameter parameter efficient fine tuning methods and adapter based fine tuning methods. \cite{ma2024segment}, ~\cite{zhang2023customized}, ~\cite{wu2023medical}. 
% % low-rank-based fine-tuning strategy 
% % First line of research focuses on the adaptability of SAM everything mode to medical image segmentation. Specifically, MedSAM ~\cite{ma2024segment} fine-tune the SAM mask decoder on a large-scaled datasets, SAMed ~\cite{}
% % [29] adopt low-rank-based fine-tuning strategy (LoRA) ~\cite{zhang2023customized} and train a default prompt for all image in the dataset, Medical SAM Adapter (MSA) [28] use adapter modules for fine-tuning
% % One line of work for SAM with medical imag segmentation focuses on % SAM has been used for medical image segmentation using conventional or parameter-efficient fine-tuning (PEFT) approaches ~\cite{ma2024segment} , ~\cite{cai2020few}, ~\cite{wu2023medical}, ~\cite{zhang2023customized}. While these methods yield satisfactory results, they still need substantial data for fine-tuning, which is not readily available in the medical domain. Moreover, these approaches do not focus on a specific region of interest (ROI) segmentation. Rather, they highlight the potential of SAM for segmenting all the regions in the medical imaging.
% % % predominantly utilized SAM's \textit{everything mode} to segment all regions in medical images. 
% % Despite it potential, its usefulness is in medical imaging is limited ~\cite{ma2024segment} as the identified regions lack semantic labels as shown in \cref{fig:sam_modes}(b). Moreover, the  clinicians primarily need to focus on specific region in the images such as the liver, kidneys, spleen, lesions, etc. 
% % Thus to get the region of interstet prompts are require. 
% % SAM [27] demonstrates in-context learning through interactive segmentation, using diverse visual
% % prompts like points, boxes, and masks, although it is limited to class-agnostic mask prediction.
% % % Therefore, the promptable mode is better suited for medical tasks because it allows for more precise segmentation, which is often needed in medical imaging. 
% % % The performance of SAM is highly dependant on the types of prompts being used. Even in some of the cases the 
% % M is exceptional in the segmenting but lacks the capability to recognize the segments it identifies.
% % We propose to employ SAM' everything mode and promptable mode together. To best of our knowledge we are first to explore the use of segment anything mode to aid the prompt generation process for medical image segmentation with SAM. 


% % The majority of these studies have focused on utilizing SAM's everything mode to generate region proposals encompassing all elements within an image,, aiming to assess SAM's suitability for medical applications. While it shows SAM's potential for medical doamin, this approach has limited applicability in the medical domain a) since these proposals lack semantic labels.

% % % Majority of these works focused on SAM' everything mode to generate region proposals of everthing in image to evaluate the applicability of SAM in medical domain. 
% % However, this approach has limited applicability in the medical domain a) since these proposals lack semantic labels, b) Clinicians primarily concentrate on meaningful regions of rnterest (ROIs) such as the liver, kidneys, spleen, and lesions.


% % It has limited applications in in medical domain as these propsals have no semantic labels and clinicians mainly focus on meaningful ROIs in clinical scenarios, e.g., the liver, kidneys, spleen, and lesions ~\cite{ma2024segment}.

% % Multiple works have used conventioanl fine-tuning or parameter-efficient fine-tuning (PEFT) of pre-trained SAM, they still require substantial data for fine-tuning. Moreover, these methods have focused mainy on SAM's everything mode, which has limited use in medical domain. On the one hand, the segmentation results do not have semantic labels. On the other hand, clinicians mainly focus on meaningful ROIs in clinical scenarios, e.g., the liver, kidneys, spleen, and lesions ~\cite{ma2024segment}.


% % % Although SAM excels in natural images, several recent studies (Deng et al., 2023; Roy et al., 2023; He et al., 2023) indicate its subpar performance in medical image segmentation tasks. Despite its subpar performance on many medical image segmentation tasks, SAM simultaneously showcases its potential through fine-tuning
% % % techniques.
% % % Training or fine-tuning large foundation models, such as SAM, from scratch poses challenges due to constraints in computing resources and data availability. While multiple works have embraced parameter-efficient fine-tuning of pre-trained SAM, they still require substantial data for supervised fine-tuning. Moreover, everything mode has limited use in medical domain because of two main reasons. On the one hand, the segmentation results do not have semantic labels. On the other hand, clinicians mainly focus on meaningful ROIs in clinical scenarios, e.g., the liver, kidneys, spleen, and lesions \cite{ma2024segment}.


% % % by sampling a grid-wise set of keypoints over the image. Subsequently, SAM generates the multiple masks when prompted by these grid-wise keypoints


% % Multiple  works have adpoted parameter-efficetn fine tuning of pre-trained SAM. However, these SAM-based works still needs large amounts of data to fine-tune the model in a supervised way, yet have not fully leverage the prompting ability.

% % Despite the MedSAM, you still need promots. 


% % Multiple previous works [16, 28, 29] have fine-tuned SAM on medical datasets. Specifically, MedSAM [16] fine-tune the SAM mask decoder on a large-scaled datasets, SAMed [29] adopt low-rank-based fine-tuning strategy (LoRA) [10] and train a default prompt for all image in the dataset, Medical SAM Adapter (MSA) [28] use adapter modules for fine-tuning. These methods yield satisfactory results, getting close to or even outperforming SOTA fully-supervised models. 


% %  Instead of directly fine-tuning a large number of parameters of the whole SAM, an alternative flexible way is to fine-tune a portion of SAM’s parameter or utilize
% % parameter-efficient fine-tuning (PEFT) techniques [4–8], in
% % order to transfer the pre-trained SAM to a specific medical
% % image segmentation task.



% % % The latter 
% % %  Specifically, we prompted the model with a
% % % 32×32 regular grid of points and for each point predicted
% % % a set of masks that may correspond to valid objects. With
% % % the ambiguity-aware model, if a point lies on a part or subpart, our model will return the subpart, part, and whole object. 
% % % where the goal is to return a valid segmentation mask given any segmentation prompt (see Fig. 1a). A
% % % prompt simply specifies what to segment in an image, e.g.,
% % % a prompt can include spatial or text information identifying
% % % an object.
% % %  The biggest highlight of SAM is
% % % its good zero-shot segmentation performance for unseen datasets and
% % % tasks. This process is driven by different prompts, e.g., points and boxes,
% % % for indicating the pixel-level semantics and region-level positions of the
% % % target objects. I
% % It is designed to segment an object through interactive prompts. Prompts can be a single point, a set of points (including an entire mask), a bounding box, or text \cite{mazurowski2023segment}.
% % It has two modes: segment everything and promptable segmentation mode. The former mode can propose an extremely exhaustive prediction of almost any object of parts on the images taken a grid-wise set of keypoints as inputs. Then the mask is generated through SAM prompted by the grid-wise keypoints. 




% % However, such segmentation results have limited use in medical domain because of two main reasons. On the one hand, the segmentation results do not have semantic labels. On the other hand, clinicians mainly focus on meaningful ROIs in clinical scenarios, e.g., the liver, kidneys, spleen, and lesions \cite{ma2024segment}.

% % and prompting objectives that typically do not require traditional supervised training labels. 



% % Due to their remarkable capabilities in transferring to multiple downstream tasks with limited training data, these models can act as foundation models with exceptional generalization abilities, and prompts play a crucial role in determining their overall performances.

% % These challenges could be significantly mitigated with the advent of foundation models (Zhou et al., 2023) and zero-shot learning (Chen et al., 2021).


% %  These models benefit from a
% % vast amount of training data and parameters, demonstrating effective performance [34, 15, 51]. 



% % The advent of Vision-Language Models (VLMs) have significantly transformed the realm of vision-related tasks, ~\cite{li2021align}, ~\cite{radford2021learning}, ~\cite{alayrac2022flamingo}. Their performance is attributed to significantly vast amount of training data they have been trained on. 

% %and parameters, demonstrating powerful performance in the training offundamental visual model backbones [34, 15, 51]. 

% % The  Segment Anything Model (SAM) is a "promptable" foundation model, trained on over 1 billion annotations, predominantly for natural images \cite{kirillov2023segment}. SAM is designed to segment an object through interactive prompts.Prompts can take the form of a single point, a set of points (including an entire mask), a bounding box, or text \cite{mazurowski2023segment}.



% % SAM is designed to require a prompt or a set of prompts to produce a segmentation mask. Technically, the model can be run without a prompt to provide any visible object, but we do not expect this to be
% % useful for medical images, where there are often many other objects in
% % the image beside the one of interest \cite{}.



% % of interest in an image given certain prompts provided by a user.

% % It  has been trained with a massive dataset of mask labels, making it highly adaptable to a wide range of downstream tasks through interactive prompts.

% % that is intended to segment user-defined objects of interest in an interactive manner. 

% % One prominent large foundation model in computer vision, the Segment Anything Model (SAM) [14].  SAM is a universal
% % segmentation model that utilizes the capabilities of ”prompting”
% % for image segmentation. SAM is trained on the Segment Anything
% % 1-Billion mask dataset (SA-1B),


% % The recently developed Segment
% % Anything Model is a foundation model that has achieved promising
% % zero-shot segmentation performance on a variety of natural image
% % datasets

% % These models benefit from a
% % vast amount of training data and parameters, demonstrating powerful performance in the training of
% % fundamental visual model backbones [34, 15, 51]. Inspired bu this, 

% % The emergence of large language models such as ChatGPT and
% % GPT-3 has sparked a new era in natural language processing (NLP),
% % characterized by their remarkable zero-shot and few-shot generalization abilities. This progress has inspired researchers to develop similarly
% % large-scale foundational models for computer vision (CV). 


% % The Segment Anything Model (SAM)  is a foundation model trained on over 1 billion annotations, predominantly for natural images ~\cite{kirillov2023segment}, . It is designed to interactively segment objects of interest as defined by the user
% %-------------------------------------------------------------------------
% \section{Related Work}
% % \subsection{Vision Language Models}
% \subsection{Segment Anything}
% % \subsection{Prompt learning}
%  \subsection{CLIP}
% \subsection{Part based segmentation}


% % All manuscripts must be in English.

% % \subsection{Dual submission}

% % Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% % discussion of the policy on dual submissions.

% % \subsection{Paper length}
% % Papers, excluding the references section, must be no longer than eight pages in length.
% % The references section will not be included in the page count, and there is no limit on the length of the references section.
% % For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% % {\bf There will be no extra page charges for \confName\ \confYear.}

% % Overlength papers will simply not be reviewed.
% % This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% % Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% % The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% % The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% % %-------------------------------------------------------------------------
% % \subsection{The ruler}
% % The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% % The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% % If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% % The presence or absence of the ruler should not change the appearance of any other content on the page.
% % The camera-ready copy should not contain a ruler.
% % (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% % Reviewers:
% % note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% % Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% % \subsection{Paper ID}
% % Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% % If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% % \subsection{Mathematics}

% % Please number all of your sections and displayed equations as in these examples:
% % \begin{equation}
% %   E = m\cdot c^2
% %   \label{eq:important}
% % \end{equation}
% % and
% % \begin{equation}
% %   v = a\cdot t.
% %   \label{eq:also-important}
% % \end{equation}
% % It is important for readers to be able to refer to any particular equation.
% % Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% % It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% % (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% % All authors will benefit from reading Mermin's description of how to write mathematics:
% % \url{http://www.pamitc.org/documents/mermin.pdf}.

% % \subsection{Blind review}

% % Many authors misunderstand the concept of anonymizing for blind review.
% % Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% % Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% % That is all.
% % (But see below for tech reports.)

% % Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% % it says that you are building on her work.
% % If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% % An example of a bad paper just asking to be rejected:
% % \begin{quote}
% % \begin{center}
% %     An analysis of the frobnicatable foo filter.
% % \end{center}

% %    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
% %    Why the previous paper was accepted without this analysis is beyond me.

% %    [1] Removed for blind review
% % \end{quote}


% % An example of an acceptable paper:
% % \begin{quote}
% % \begin{center}
% %      An analysis of the frobnicatable foo filter.
% % \end{center}

% %    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
% %    Why the previous paper was accepted without this analysis is beyond me.

% %    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% % \end{quote}

% % If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% % In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% % \begin{quote}
% % [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% % \end{quote}

% % Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% % For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% % Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% % Then submit the tech report as supplemental material.
% % Again, you may not assume the reviewers will read this material.

% % Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% % For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% % solution.
% % The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% % You can handle this paper like any other.
% % Do not write ``We show how to improve our previous work [Anonymous, 1968].
% % This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% % That would be silly, and would immediately identify the authors.
% % Instead write the following:
% % \begin{quotation}
% % \noindent
% %    We describe a system for zero-g frobnication.
% %    This system is new because it handles the following cases:
% %    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
% %    Ours handles it by including a foo term in the bar integral.

% %    ...

% %    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
% %    It displayed the following behaviours, which show how well we solved cases A and B: ...
% % \end{quotation}
% % As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% % A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% % He or she would have to be sure that no other authors could have been contracted to solve problem B.
% % \medskip

% % \noindent
% % FAQ\medskip\\
% % {\bf Q:} Are acknowledgements OK?\\
% % {\bf A:} No.  Leave them for the final copy.\medskip\\
% % {\bf Q:} How do I cite my results reported in open challenges?
% % {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% % For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% % Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% % \begin{figure}[t]
% %   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% %    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

% %    \caption{Example of caption.
% %    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
% %    \label{fig:onecol}
% % \end{figure}

% % \subsection{Miscellaneous}

% % \noindent
% % Compare the following:\\
% % \begin{tabular}{ll}
% %  \verb'$conf_a$' &  $conf_a$ \\
% %  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% % \end{tabular}\\
% % See The \TeX book, p165.

% % The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% % So \eg is correct, {\em e.g.} is not.
% % The provided \verb'\eg' macro takes care of this.

% % When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% % If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% % However, use it only when there are three or more authors.
% % Thus, the following is correct:
% %    ``Frobnication has been trendy lately.
% %    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
% %    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% % This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% % \begin{figure*}
% %   \centering
% %   \begin{subfigure}{0.68\linewidth}
% %     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% %     \caption{An example of a subfigure.}
% %     \label{fig:short-a}
% %   \end{subfigure}
% %   \hfill
% %   \begin{subfigure}{0.28\linewidth}
% %     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% %     \caption{Another example of a subfigure.}
% %     \label{fig:short-b}
% %   \end{subfigure}
% %   \caption{Example of a short caption, which should be centered.}
% %   \label{fig:short}
% % \end{figure*}

